DSRM: Boost Textual Adversarial Training with Distribution Shift Risk Minimization

Adversarial training is one of the best-performing methods in improving the robustness of deep language models. However, robust models come at the cost of high time consumption, as they require multi-step gradient ascents or word substitutions to obtain adversarial samples. In addition, these generated samples are deficient in grammatical quality and semantic consistency, which impairs the effectiveness of adversarial training. To address these problems, we introduce a novel, effective procedure for instead adversarial training with only clean data. Our procedure, distribution shift risk minimization (DSRM), estimates the adversarial loss by perturbing the input data's probability distribution rather than their embeddings. This formulation results in a robust model that minimizes the expected global loss under adversarial attacks. Our approach requires zero adversarial samples for training and reduces time consumption by up to 70\% compared to current best-performing adversarial training methods. Experiments demonstrate that DSRM considerably improves BERT's resistance to textual adversarial attacks and achieves state-of-the-art robust accuracy on various benchmarks.

==> outline/3analysis.tex <==
\section{Trade-offs in Standard Adversarial Training}
This section discusses the trade-off between computational costs and performance in constructing robust language models. We empirically show that larger perturbation radii and steps enhance the effectiveness of textual adversarial training. Similar phenomena are previously found in image datasets by 
\citet{zhang2019theoretically} and \citet{gowal2020uncovering}. The experimental results for these two modifications are shown in Figure \ref{fig: analysis}.

% 1. 更大的步数能提升效果
% 2. 省略对范数的约束能提升效果
\begin{figure}[t]
 \centering
 \subfigure[]{
  \begin{minipage}[b]{0.225\textwidth}
   \includegraphics[width=1\textwidth]{Figures/norm_1.pdf}
  \end{minipage}
 }
     \subfigure[]{
      \begin{minipage}[b]{0.226\textwidth}
       \includegraphics[width=1\textwidth]{Figures/step_2.pdf}
      \end{minipage}
     }
 \caption{The impact of different values of the perturbation threshold (a) and ascent steps (b) on the IMDB dataset. We show the accuracy score of the FreeLB \cite{zhu2020freelb} algorithm under three attack methods. Sub-figure (a) uses a 10-step gradient ascent with different constraints on the $l_{2}$ norm of perturbations. In sub-figure (b), each step introduces a perturbation of length 0.05.}
\vspace{-1mm}
\label{fig: analysis}
\end{figure}


In sub-figure (a), relaxing the perturbation threshold increases the model robustness remarkably under the attack of Textfooler and BertAttack. Only a slight decrease occurs when the threshold is larger than 0.6 for Textbugger. A wide threshold is equivalent to removing the projection at the norm constraint and achieves better performance relative to small perturbations.

In subfigure (b), as the value of steps grows, the models' accuracy under attack increases until they reach their peak points. Subsequently, they begin to decline as the number of steps increases consistently. Notably, the optimal results are 4-10\% higher in (b) relative to (a), demonstrating that a larger number of steps is beneficial to improve the effectiveness of the adversarial training.

Here is a possible explanation for the above performance. We describe the standard adversarial training as exploring potential adversarial samples in the embedding space. When the step number is small, the adversarial sample space is correspondingly simple, causing the model to underestimate the adversarial risks. Such rudimentary models exhibit poor defensive capabilities when a high-intensity attack arrives. A broader search interval can prevent these defects and achieve outstanding robustness as the number of steps grows.

However, these results occur late in the step growth process. As shown in (b), a defence model needs 30 steps (about ten times the time cost) for Textfooler, 20 for Textbugger, and 40 for BertAttack to achieve optimal performance. This drawback considerably reduces the efficiency and practicality of adversarial training. We further analyse the time consumption in section \ref{sec:time}. To address the above trade-off problem, we propose estimating the adversarial risk by perturbing the distribution of clean data. Our approach omits the multi-step search process for optimal perturbation and requires only training samples. We detail our theoretical framework in the next section.

% We give a possible explanation for the above performance. We describe the standard adversarial training as an exploration of potential adversarial samples in the embedding space. When the step number is small, the adversarial sample space is correspondingly simple, causing the model to underestimate the adversarial risks. Such rudimentary models exhibit poor defensive capabilities when a high-intensity attack arrives. This defect can be gradually avoided when the number of steps becomes larger, which explains the increase in model robustness as the number of steps grows. When the number of steps exceeds the optimal threshold, excessive focus on adversarial samples that are not similar to the original samples induces a decline in both model accuracy and robustness.




